Delay Analysis of Multichannel Parallel Contention Tree Algorithms (MP-CTA)

Contention tree algorithm is initially invented as a solution to improve the stable throughput problem of Slotted ALOHA in multiple access schemes. Even though the throughput is stabilized in tree algorithms, the delay of requests may grow to infinity with respect to the arrival rate of the system. Delay depends heavily on the exploration of the tree structure, i.e., breadth search, or depth search. Breadth search is necessary for faster exploration of tree. The analytical probability distribution of delay, which is available mostly for depth search, is not generalizable to all breadth search. In this paper we fill this gap through though arbitrary grouping of branches and including this in the delay analysis. This enables obtaining the delay analysis of any contention tree algorithm that runs a breadth first search exploration. We show through simulations that the analysis is in agreement with the realizations.

==> original_delay_analysis.tex <==
\subsection{Access delay}
\label{ramalamadindon}
In this section, we address the derivation of the statistics of the access delay of a multichannel tree, which will henceforth be modeled by the random variable $\Theta_N$, provided $N$ initial contenders. After the analysis of $\mathcal{T}_N$, we have many of the tools that we require in order to characterize this new variable.

Since the access delay is usually more relevant than the length of the tree, it is worth addressing the calculation of the mean value of $\Theta_N$ separately. After this, the complete characterization of this random variable will be obtained by means of its PMF.
\subsubsection{Average}
We define the access delay $\Theta_N$ of a focused, single device as the number of time slots between its first transmission and its successful transmission. Since the first slot of a tree is always a collision, the access delay varies between 1 slot (if the device transmits in the second slot) and $\mathcal{L}_N-1$ (if the device transmits in the last slot), where  $\mathcal{L}_N$ is the random variable modeling the number of nodes contained in a tree, i.e., the length of the equivalent single channel tree.
In order to compute the average of $\Theta_N$, we introduce the auxiliary variable $\mathcal{H}_N$, which denotes the number of levels of the tree that the device has traversed before its successful transmission. The PMF of $\mathcal{H}_N$ was given in \cite{janssenjong} as:
\begin{equation}
	p_{\mathcal{H}_N}(h) \triangleq \Pr\left\lbrace \mathcal{H}_N = h \right\rbrace
 = \left(1-\frac{1}{2^h}\right)^{n-1} \!\!\!\!- \left(1-\frac{1}{2^{h-1}}\right)^{n-1}.
 \label{walkthisway}
\end{equation}
By applying the law of total expectation, we can calculate the mean of $\Theta_N$ as:
\begin{equation}
\mathrm{E}\{\Theta_N\} = \sum_{h=1}^\infty\mathrm{E}\left\lbrace\Theta_N \, \big| \, \mathcal{H}_N = h\right\rbrace \cdot p_{\mathcal{H}_N}(h).
\label{ificouldfly}
\end{equation}
Notice that the summation above starts with $h=1$, since it is not possible to successfully transmit at the level 0. The only unknown in this expression is $\mathrm{E}\left\lbrace\Theta_N  | \mathcal{H}_N = h\right\rbrace$, which is the average delay experienced by a device provided that it has successfully transmitted at the level $h$. For a more convenient notation, let us introduce $\Theta_N^h$, defined as the random variable modeling the access delay of a device that has successfully transmitted at the level $h$:
\begin{equation}
\Theta_N^h \triangleq \Theta_N \big| _{\mathcal{H}_N = h}.
\label{defidefi}
\end{equation}
After using this new definition, \eqref{ificouldfly} becomes:
\begin{equation}
\mathrm{E}\{\Theta_N\} = \sum_{h=1}^\infty\mathrm{E}\left\lbrace\Theta_N^h\right\rbrace \cdot p_{\mathcal{H}_N}(h).
\label{crowdchant}
\end{equation}
At this point, let us define $\Omega_N^h$ as the position of the slot at the level $h$ in which the device successfully transmitted, assuming that the slots within a certain level are numbered according to their transmission order. In other words, $\Omega_N^h$ is the number of slots that are transmitted from the first slot belonging to the level $h$ until the slot containing the successful transmission of our focused device, both inclusive. By using this variable, we can decompose $\Theta_N^h$ as follows:
\begin{equation}
\Theta_N^h = \begin{cases}
1 & \text{if }h = 1,\\
\mathcal{S}_N^{h-1} + \Omega_N^h  & \text{if }h > 1,
\end{cases}
\label{sambapati}
\end{equation}
where $\mathcal{S}_N^{h-1}$ was defined in \eqref{ajvar} as the partial sum of the number of slots between levels $0$ and $h-1$.
\begin{figure}
	\centering
	\includegraphics[]{img/delay_explanation}
	\caption{Example of tree depicting the variables $\mathcal{S}_N^{h-1}$ and $\Omega_N^h$, given a focused device (in green) that successfully transmits at the level $m=4$.}
	\label{fig:delay_explanation}
\end{figure}
The meaning of this problem is illustrated in Fig. \ref{fig:delay_explanation}, where our focused device has transmitted in the second slot of the fourth level, so that we can compute the access delay that it has experienced by counting the number of slots up to level 3 ($\mathcal{S}_N^{h-1} = 5$ slots) and then the number of slots within the level 4 ($\Omega_N^h = 2$ slots).

If we apply the expectation operator in \eqref{sambapati}, we obtain the following expressions for $h >1$:
\begin{align}
\mathrm{E}\{\Theta_N^h\} &= \mathrm{E}\left\lbrace\mathcal{S}_N^{h-1}\right\rbrace + \mathrm{E}\left\lbrace\Omega_N^h\right\rbrace\\
&= \sum_{k = 1}^{h-1}\mathrm{E}\left\lbrace\mathcal{T}_N^{k}\right\rbrace + \mathrm{E}\left\lbrace\Omega_N^h\right\rbrace\\
&= \sum_{k = 0}^{h-2}\mathrm{E}\left\lbrace\left\lceil\frac{\mathcal{X}_N^{k}}{G}\right\rceil\right\rbrace + \mathrm{E}\left\lbrace\Omega_N^h\right\rbrace\\
&= \sum_{k = 0}^{h-2}\sum_{x_k = 1}^{\hat{X}} \left\lceil \frac{x_k}{G} \right\rceil \Pr\left\lbrace \mathcal{X}_N^{k} = x_k \right\rbrace + \mathrm{E}\left\lbrace\Omega_N^h\right\rbrace
\label{wellalright}
\end{align}
The probability in \eqref{wellalright} can be obtained as a modified version of the probability calculated in \cite{bianchi}: 
\begin{equation}
\Pr\{ \mathcal{X}_N^m = x \} = \sum_{i = x}^{\min\left( N-x,R \right)} \frac{\Psi_{i,x}^N {R\choose{i}} i!}{R^N},
\label{lamia}
\end{equation}
Therefore, only the  of an expression for  $\mathrm{E}\left\lbrace\Omega_N^h\right\rbrace$ is needed. In order to do so, let us define $\Lambda_N^h$ as the random variable modeling the number of nodes that lie between the first node belonging to the level $h$ and the node containing the successful transmission of the device, both inclusive. In other words, $\Lambda_N^h$ reflects the position of the node of the successful transmission at the level $h$. In our example of Fig. \ref{fig:delay_explanation}, $\Lambda_N^h = 8$ nodes, since the successful transmission took place in the eighth node of level $h = 4$. From this definition it follows that:
\begin{equation}
\Omega_N^h = \left\lceil \frac{\Lambda_N^h}{2 G} \right\rceil.
\end{equation}
After applying the expectation operator, the average of $\Omega_N^h$ turns out to be:
\begin{equation}
\mathrm{E}\left\lbrace\Omega_N^h\right\rbrace = \sum_{\lambda_h=1}^{\min(N,2^h)} \left\lceil \frac{\lambda_h}{2 G} \right\rceil \cdot \Pr\left\lbrace\Lambda_N^{h} = \lambda_h\right\rbrace.
\label{ybicarbonato}
\end{equation}
Therefore, the PMF of $\Lambda_N^h$ is required to continue. 

An unbiased binary tree is statistically symmetrical, i.e. it is equally probable for a device to transmit in any node of a given level. Hence it is clear that $\Lambda_N^h$ follows an uniform distribution ranging from 1 to the total number of nodes $\mathcal{L}_N^h$ at the level $h$:
\begin{equation}
	\Lambda_N^h \sim U(1,\mathcal{L}_N^h).
\end{equation}
Since $\mathcal{L}_N^h$, the upper limit of $\Lambda_N^h$, is itself a random variable, we need to apply the law of total probability to take into account every possible value.
%\begin{align}
%\mathrm{E} \left\lbrace \Lambda_N^h \right\rbrace &= \sum_{l_h = 1}^{\infty} \mathrm{E} \left\lbrace \Lambda_N^h | \, \mathcal{L}_N^h = l_h\right\rbrace \cdot \Pr \left\lbrace \mathcal{L}_N^h = l_h\right\rbrace\\
%&= \sum_{l_h = 1}^{\infty} \frac{l_h + 1}{2} \cdot \Pr \left\lbrace \mathcal{L}_N^h = l_h\right\rbrace. \label{europa}
%\end{align}
%The upper bound of these summations may be alternatively set to $\min\left(\frac{N}{2}, 2^{h-1}\right)$ instead of $\infty$, since the possible number of nodes in a certain level is limited by the number of contenders and the level index. However, $\infty$ is preferred here to lighten the notation.
%
%As every collision at the level $m-1$ generates two new nodes at the level $h$, the PMF of $\mathcal{L}_N^h$ can be related with the PMF of $\mathcal{X}_N^{h-1}$ as follows:
%Therefore, after combining \eqref{europa} and \eqref{treat} we obtain:
%\begin{align}
%\mathrm{E} \left\lbrace \Lambda_N^h \right\rbrace &= \sum_{x = 1}^{\infty} \frac{2 x + 1}{2} \cdot \Pr \left\lbrace \mathcal{X}_N^{h-1} = x\right\rbrace\\
%&= \mathrm{E} \left\lbrace \mathcal{X}_N^{h-1} \right\rbrace + \frac{1}{2}
%\end{align}
%
%Regarding the PMF of $\Lambda_N^h$, we use the law of total probability in a similar manner:
\begin{equation}
\Pr \left\lbrace \Lambda_N^h = \lambda_h \right\rbrace =  \sum_{l_h = 1}^{\infty}  \Pr \left\lbrace \Lambda_N^h =\lambda_h \, | \, \mathcal{L}_N^h = l_h\right\rbrace \cdot \Pr \left\lbrace \mathcal{L}_N^h = l_h\right\rbrace \label{soulsacrifice}
\end{equation}
As $\Lambda_N^h$ is an uniform random variable, the probability of any value is constant, provided a deterministic upper bound. Therefore it follows that:
\begin{equation}
\Pr \left\lbrace \Lambda_N^h =\lambda_h \, | \, \mathcal{L}_N^h = l_h\right\rbrace = \begin{cases}
\frac{1}{l_h} & \text{if } 1 \leq \lambda_h \leq l_h,\\
0 & \text{otherwise.}
\end{cases} \label{jingo}
\end{equation}
The probability of obtaining $l_h$ nodes at the level $h$ can be derived directly from the number of collisions in the previous level. However, since we are assuming that the successful transmission of our focused device occurred at the level $h$, we need to normalize the probability of a certain number of collisions to leave out the possibility of no collisions. Furthermore, it is clear that only even values of $l_h$ are allowed. Thus, the final expression of the probability of $l_h$ nodes at the level $h$ is:  
\begin{equation}
\Pr \left\lbrace \mathcal{L}_N^h = l_h\right\rbrace = \begin{cases}
\frac{\Pr \left\lbrace \mathcal{X}_N^{h-1} = \frac{l_h}{2} \right\rbrace}{1-\Pr \left\lbrace \mathcal{X}_N^{h-1} = 0 \right\rbrace} & \text{if $l_h$ even,} \\
0 & \text{if $l_h$ odd.}
\end{cases} \label{treat}
\end{equation}
After combining \eqref{soulsacrifice}, \eqref{jingo} and \eqref{treat}, the final expression for the PMF of $\Lambda_N^h$ is obtained:
\begin{equation}
\Pr \left\lbrace \Lambda_N^h = \lambda_h \right\rbrace= \sum_{l_h = \lambda_h}^{\infty} \frac{\Pr \left\lbrace \mathcal{L}_N^h = l_h\right\rbrace}{l_h}\\= \sum_{x = \left\lceil \!\frac{\lambda_h}{2}\!\right\rceil}^{\infty} \frac{\Pr \left\lbrace \mathcal{X}_N^{h-1} = x \right\rbrace}{2 x \left(1-\Pr \left\lbrace \mathcal{X}_N^{h-1} = 0 \right\rbrace\right)}.
\end{equation}
After replacing this intermediate result in \eqref{ybicarbonato}, we obtain the final expression of the average of $\Omega_N^h$:
\begin{equation}
\mathrm{E}\left\lbrace\Omega_N^h\right\rbrace = \sum_{\lambda_h=1}^{\min(N,2^h)} \left\lceil \frac{\lambda_h}{2 G} \right\rceil \sum_{x = \left\lceil \!\frac{\lambda_h}{2}\!\right\rceil}^{\infty} \frac{\Pr \left\lbrace \mathcal{X}_N^{h-1} = x \right\rbrace}{2 x}.
\label{sharpdressedman}
\end{equation}
Finally, we just need to combine \eqref{crowdchant} and \eqref{wellalright} to obtain the expression for the average of $\Theta_N$:
\begin{equation}
\mathrm{E}\{\Theta_N\} =\sum_{k = 0}^{h-2} \!\!\left(\!\sum_{x_k = 1}^{\hat{X}} \!\left\lceil \frac{x_k}{G} \right\rceil\! \Pr\left\lbrace \mathcal{X}_N^{k} = x_k \right\rbrace\! +\! \mathrm{E}\left\lbrace\Omega_N^h\right\rbrace\!\right) \!\cdot p_{\mathcal{H}_N}(h)\!.
\end{equation}
$\Pr\left\lbrace \mathcal{X}_N^{k} = x_k \right\rbrace$ is obtained from \eqref{lamia}, $\mathrm{E}\left\lbrace\Omega_N^h\right\rbrace$ from \eqref{sharpdressedman}, and $ p_{\mathcal{H}_N}(h)$ from \eqref{walkthisway}.

\subsubsection{Probability mass function}
As it was done in the derivation of the PMF of the number of required time slots, this section is divided in two parts. First, the details of the derivation of the PMF are explained. At the end of the section, a summary with the most important steps in the derivation is presented, along with a table compiling the variables that were used in the process.
\paragraph{Derivation approach}
The goal of this section is to derive an expression for the PMF of $\Theta_N$, which is formally defined as:
\begin{equation}
p_{\Theta_N}(\theta) \triangleq \Pr\left\lbrace\Theta_N = \theta \right\rbrace \\
\label{legs}
\end{equation}
We can benefit from the law of total probability and the definition provided in \eqref{defidefi} to reformulate our problem as follows:
\begin{equation}
p_{\Theta_N}(\theta) =\sum_{h=1}^\infty \Pr\left\lbrace\Theta_N^h = \theta \right\rbrace \cdot p_{\mathcal{H}_N}(h).
\label{gimmeallyourlovin}
\end{equation}
Hence, we need to obtain the probability $p_{\Theta_N^h}(\theta_h)$ that our focused device successfully transmits with delay $\theta_h$, given the knowledge that it has transmitted at the level $h$:
\begin{equation}
p_{\Theta_N^h}(\theta_h) \triangleq \Pr\left\lbrace\Theta_N^h = \theta_h \right\rbrace.
\end{equation}
The variable $\Theta_N^h$ was defined in \eqref{sambapati} as the sum of ${S}_N^{h-1}$ and  $\Omega_N^h$ for $h>1$. Again, we face the problem of obtaining the PMF of the sum of two dependent random variables. As in the previous section, this is accomplished by means of their joint PMF:
\begin{equation}
p_{\Theta_N^h}(\theta_h) = \sum_{\omega_{h}=1}^{\left\lceil \frac{2^h}{2G} \right\rceil} p_{\Omega_N^h, \mathcal{S}_N^{h-1}} (\omega_{h},\theta_h - \omega_{h}).
\label{spinachs}
\end{equation}
The upper limit of the summation represents the maximum number of slots that can be obtained at the level $h$. At this point, the problem is to derive the joint PMF of $\mathcal{S}_N^{h-1}$ and $\Omega_N^h$. The law of total probability can be applied to introduce $\mathcal{T}_N^{h}$, which provides information about the number of slots at the level $h$. This is useful in order to infer the probability of transmitting at position $\Omega_N^h = \omega_h$.
\begin{equation}
p_{ \Omega_N^h, \mathcal{S}_N^{h-1}} (\omega_h, s_{h-1}) = \sum_{t_h} p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | t_h, s_{h-1}) \cdot p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1}).
\label{fries}
\end{equation}

The second term in the right-hand side of this equation is already known if $p_{\mathcal{T}_N(t)}(t)$ has been computed first, as it was derived in \eqref{currywurst} in Appendix \ref{LEL}. Therefore, we need to calculate only the first term, which is the probability of transmitting in the position $\omega_h$ out of $t_h$ slots at the level $h$, provided that the length of the tree so far is $s_{h-1}$.

If the tree is unbiased, as we have assumed for the whole analysis, all nodes within a tree are equally like, since the tree is statistically symmetrical. Therefore, if $G = 1$, every slot is equally likely, since they all contain two nodes. Thus, the desired probability in that case is:
\begin{equation}
p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}}(\omega_h | t_h, s_{h-1}) = \frac{1}{t_h}.
\end{equation}
%\begin{align}
%p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} &(\omega_h | t_h, s_{h-1}) = \nonumber\\ &=p_{\Omega_N^h | \mathcal{L}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | 2 t_h, s_{h-1}) \\&= \frac{1}{t_h}.
%\end{align}
Intuitively, the probability to transmit in a certain position given $t_h$ options is just $\frac{1}{t_h}$, as long as all options are equally likely. This means that, if $G = 1$:
\begin{equation}
p_{ \Omega_N^h, \mathcal{S}_N^{h-1}} (\omega_h, s_{h-1}) = \sum_{t_h} \frac{ p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1})}{t_h}.
\label{sensi}
\end{equation}
However, in the case of $G > 1$, the number of nodes in one slot is not fixed, but it ranges from 2 to $2 G$ nodes. Namely, given $l_h$ nodes at the level $h$ that are grouped into $t_h$ slots, there will be $t_h -1$ slots of size $2 G$ and one (the last one) of size $l_h - 2 G (t_h-1)$. This difference in the size of the slots produces an asymmetry in the tree: it is less probable to transmit in the last slot than in the rest of them. In order to cope with this asymmetry, let us introduce the number of nodes $\mathcal{L}_N^h$ at the level $h$ into the problem, with the help of the law of total probability:
\begin{equation}
p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | t_h, s_{h-1}) = 
 \sum_{l_h} p_{\Omega_N^h | \mathcal{L}_N^h, \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | l_h, t_h, s_{h-1}) \cdot p_{\mathcal{L}_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (l_h | t_h, s_{h-1}).
\label{pizza}
\end{equation}
In the first term of \eqref{pizza}, the simplification 
\begin{equation}
p_{\Omega_N^h | \mathcal{L}_N^h, \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | l_h, t_h, s_{h-1}) = p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h)
\end{equation}
may be applied, since it is clear that the probability of transmitting in the slot $\omega_h$ is only influenced by the number of nodes $l_h$ at the level $h$. In the second term, the Bayes' theorem may be applied with the intention of changing the order of the variables. After such manipulations, the following expression is obtained:
\begin{equation}
p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | t_h, s_{h-1}) = \sum_{l_h} p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h) \cdot p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1} | \mathcal{L}_N^h } (t_h, s_{h-1} | l_h)  \cdot \frac{p_{\mathcal{L}_N^h}(l_h)}{p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1})}.
\end{equation}
 As a result, we expressed 
$p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | t_h, s_{h-1})$ as a combination of four probabilities:
\begin{enumerate}
	\item The probability $p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1})$ is \eqref{currywurst}, derived in Appendix \ref{LEL}.
	\item The probability $p_{\mathcal{L}_N^h}(l_h)$ of obtaining $l_h$ nodes at the level $h$ can be calculated directly from the PMF of the number of collisions, as follows: 
	\begin{equation}
		p_{\mathcal{L}_N^h}(l_h) = p_{\mathcal{X}_N^{h-1}}\!\!\left(\frac{l_h}{2}\right).
		\label{arenques}
	\end{equation}		
	
	Note that in a binary tree only an even number of nodes is allowed at each level.
	\item The probability
	\begin{equation}
	p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1} | \mathcal{L}_N^h } (t_h, s_{h-1} | l_h)
	\label{horchatucha}
	\end{equation}
	of obtaining $t_h$ slots at the level $h$ and $s_{h-1}$ slots from level 1 to $m-1$, given $l_h$ nodes at the level $h$, has not been addressed yet.
	\item The probability
	\begin{equation}
	 p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h)
	 \label{sepiarellena}
	\end{equation}
	of transmitting in the position $\omega_h$ given $l_h$ nodes at the level $h$ has not been calculated either.
\end{enumerate}

Let us tackle \eqref{sepiarellena} first. This probability is simple to compute, since it is just the number of nodes in one slot divided by the total number of slots. However, since the last slot may have a different size with respect to the others, two cases need to be considered:
\begin{gather}
p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h) = \begin{cases}
\frac{2 G}{l_h} & \omega_h < t_h, \\
\frac{l_h - 2 G (t_h -1)}{l_h} & \omega_h = t_h,\\
0 & \omega_h > t_h,
\end{cases}
\quad\text{ where  } 	t_h =  \left\lceil \frac{l_h}{2 G} \right\rceil.
\label{cuerotroleo}
\end{gather}

%\begin{equation}

%\end{equation}

Now we are left with the problem of calculating \eqref{horchatucha}, that is, the probability of obtaining $t_h$ slots at the level $h$ and a total of $s_{h-1}$ slots from level 1 to level $m-1$, given that we have $l_h$ nodes at the level $h$. We know that the number of slots is completely determined by the number of nodes, therefore we only allow for $t_h =  \left\lceil \frac{l_h}{2 G} \right\rceil$. This condition leads to the following expression:
\begin{equation}
p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1} | \mathcal{L}_N^h } (t_h, s_{h-1} | l_h) = \begin{cases}
\frac{p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1})}{ p_{\mathcal{T}_N^h}(t_h)} & t_h = \left\lceil \frac{l_h}{2 G} \right\rceil.\\
0 & \text{otherwise.}
\end{cases}
\label{pepperoni}
\end{equation}
After combining \eqref{pizza} and \eqref{pepperoni}, the following result is obtained:
\begin{equation}
p_{\Omega_N^h | \mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (\omega_h | t_h, s_{h-1}) =  \sum_{l_h \in L_h} p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h) \cdot \frac{p_{\mathcal{L}_N^h}(l_h)}{p_{\mathcal{T}_N^h}\left(t_h \right)},
\label{ketchup}
\end{equation}
where
\begin{align}
L_h = \left\lbrace l_h \; : \; t_h = \left\lceil \frac{l_h}{2 G} \right\rceil \right\rbrace = \left\lbrace l_h \; : \; 2 (t_h-1) G < l_h \leq 2 t_h G\right\rbrace.
\end{align}

Finally, if we merge \eqref{fries} and \eqref{ketchup} we obtain the following result after some basic manipulation:
\begin{align}
p_{ \Omega_N^h, \mathcal{S}_N^{h-1}} (\omega_h, s_{h-1}) \nonumber
&= \sum_{t_h} \left( \sum_{l_h \in L_h} p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h) \cdot\frac{p_{\mathcal{L}_N^h}(l_h)}{p_{\mathcal{T}_N^h}\left( t_h \right)} \right) \cdot p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} (t_h, s_{h-1})\\
&= \sum_{l_h} p_{\Omega_N^h | \mathcal{L}_N^h} (\omega_h | l_h) \cdot p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}} \left(\left\lceil \frac{l_h}{2 G} \right\rceil, s_{h-1}\right)  \cdot \frac{p_{\mathcal{L}_N^h}(l_h)}{p_{\mathcal{T}_N^h}\left(\left\lceil \frac{l_h}{2 G} \right\rceil \right)}.
\label{pita}
\end{align}

At this point, we just need to combine \eqref{gimmeallyourlovin}, \eqref{spinachs}, and \eqref{pita} to obtain the PMF of $\Theta_N$. 
%In Fig. \ref{fig:pmfs_delay}, example PMFs of the access delay are shown for $N = 60$ and $G=\{1,...,4\}$. The strange shape of the PMF reflects the \textit{breadth-first} traversal, since every node belonging to an early level has about the same probabilities to be occupied by a successful device. In Fig. \ref{fig:cdfs_delay}, several CDFs for different values of $G$ are depicted. As it happened with the length of the tree, the average and variance of the access delay decreases when $G$ increases. 
%\begin{figure}
%\centering
%\includegraphics[width=0.5\linewidth]{img/pmfs_delay}
%\caption{Probability mass functions of the access delay experienced by a contender in a multichannel tree for several values of $G$, given $N = 60$ initial contenders.}
%\label{fig:pmfs_delay}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=0.5\linewidth]{img/cdfs_delay}
%\caption{Cumulative distribution functions of the access delay experienced by a contender in a multichannel tree for several values of $G$, given $N=60$ initial contenders.}
%\label{fig:cdfs_delay}
%\end{figure}

%Finally, in Fig. \ref{fig:99th_percentile_reliab}, the evolution of the 99th percentile of $\Theta_N$ along $G$ for several values of $N$ is presented. This kind of plot can be used for selecting the required $G$ to meet a certain delay requirement with the desired level of reliability. For example, if collisions of at most 40 contenders are expected and the maximum acceptable delay is 30 time slots, $G = 3$ is enough to meet this requirement with 99\% reliability, according to Fig. \ref{fig:99th_percentile_reliab}. If the delay requirement is instead 20 slots, the required $G$ would be $G = 5$. Other values can be selected according to the specific details of each situation. In this way, multichannel Tree Algorithms may be applied to provide guaranteed reliability in low-delay scenarios.
%\begin{figure}
%	\centering
%	\includegraphics[width=0.5\linewidth]{img/99th_percentile_reliab}
%	\caption{Value of the 99th percentile of $\Theta_N$ for several values of $N$ and $G$}
%	\label{fig:99th_percentile_reliab}
%\end{figure}


%In the light of this result, we confirm our hypothesis that multichannel Tree Algorithms can yield a lower access delay with respect to single channel Tree Algorithms, in exchange for additional resources. Thus, Tree Algorithms may be applied to multichannel scenarios where contention is expected, such as the LTE Random Access Channel, in order to provide reliability to delay sensitive devices. Depending on the application, different multichannel or single channel configurations for a Tree Algorithm can be selected in order to meet the delay requirements with an optimal use of resources.

%\paragraph{Summary} In this section, a closed-form approximate expression for the PMF $p_{\Theta_N}(\theta)$ of the access delay has been derived. As in the previous section, a single expression would be cumbersome, therefore a piecemeal approach has been again preferred.
%
%In order to summarize the whole process, the Algorithm \ref{alg:pmf_delay} shows the most important steps that are required to compute $p_{\Theta_N}(\theta)$. The process starts with the calculation of the number of considered levels $M$ to reach the desired accuracy. After that, each possible position of transmission $\omega_h$  is traversed for every considered level. If $G=1$, only a simple equation is required to compute the probability of that position, given a certain number of previous slots that is computed as $s_{h-1} = \theta - \omega_h$. Otherwise, it is necessary to go over every possible number $l_h$ of nodes at the level $h$. The next step is to compute the four different probabilities that appear in \eqref{pita} from $\theta$, $h$, $\omega_h$, and $\l_h$. After doing so, the probability of transmitted in the position $\omega_h$ given $s_{h-1}$ previous slots can be computed. Then the probability of transmitting after $\theta$ slots, assuming transmission at the level $h$ can be calculated. Finally, the law of total probability is applied to obtain the final probability of a certain access delay.

%\begin{algorithm}
%	\caption{Computation of $p_{\Theta_N}(\theta)$}
%	\label{alg:pmf_delay}
%	\begin{spacing}{1.15}
%		\begin{algorithmic}
%			\Require $p_{\mathcal{T}_N^h}(t_h)$ and $p_{\mathcal{T}_N^h, \mathcal{S}_N^{h-1}}(t_h,s_{h-1})$ from previous section
%			\State \eqref{paella} $\rightarrow$ {\small Compute $M$ according to desired accuracy}
%			\For{$1 \leq m \leq M$} 
%				\For{$1 \leq \omega_h \leq \left\lceil \frac{2^h}{2G} \right\rceil$}
%					\If{$G = 1$}
%						\State \eqref{sensi}  $\rightarrow$ {\small Pr. of transmitting in position $\omega_h$ given $s_{h-1}$ \\ \hspace{4.9em} \phantom{(00)  $\rightarrow$ }slots from levels 1 to $m-1$}
%					\Else
%						\For{$2 \leq l_h \leq N \; \wedge \; l_h$ even} 
%							\State \eqref{cuerotroleo}  $\rightarrow$ {\small Pr. of transmitting in position $\omega_h$ \\ \hspace{6.6em} \phantom{(00)  $\rightarrow$ }given $l_h$ nodes}
%							\State \eqref{currywurst}  $\rightarrow$ {\small Pr. of obtaining $\lceil l_h / 2G\rceil$ slots in the\\ \hspace{6.6em} \phantom{(00)  $\rightarrow$ }level $h$ and $s_{h-1}$ slots from levels 1 to\\ \hspace{6.6em} \phantom{(00)  $\rightarrow$ }$m-1$}
%							\State \eqref{arenques}  $\rightarrow$ {\small Pr. of obtaining $l_h$ nodes at the level $h$}
%							\State \eqref{brezen}  $\rightarrow$ {\small Pr. of obtaining $\lceil l_h / 2G\rceil$ slots in the\\ \hspace{6.6em} \phantom{(00)  $\rightarrow$ }level $h$}
%						\EndFor
%						\State \eqref{pita}  $\rightarrow$ {\small Pr. of transmitting in position $\omega_h$ given $s_{h-1}$ \\ \hspace{4.8em} \phantom{(00)  $\rightarrow$ }slots from levels 1 to $m-1$}
%					\EndIf
%				\EndFor
%				\State \eqref{spinachs}  $\rightarrow$ {\small Pr. of transmitting after $\theta$ slots, assuming \\ \hspace{1.8em} \phantom{(00)  $\rightarrow$ }transmission at the level $h$}
%			\EndFor
%			\State \eqref{gimmeallyourlovin} $\rightarrow$ {\small PMF of the access delay}
%		\end{algorithmic}
%	\end{spacing}
%\end{algorithm}
%
%\begin{table}[]
%	\centering 
%	\caption{Most relevant variables for computing $p_{\Theta_N}(\theta)$}
%	\label{hy-label}
%	\begin{tabular}{@{}cl@{}}
%		\toprule
%		\textbf{Variable} & \multicolumn{1}{c}{\textbf{Definition}}                                                                                                                                                                 \\ \midrule
%				\vspace*{2mm}
%				$\mathcal{H}_N$        & Number of levels traversed by a certain device   \\
%		\vspace*{2mm}
%		$\Theta_N$        & \begin{tabular}[c]{@{}l@{}}Number of time slots between the initial \\ collision and the successful transmission of \\ a certain device (access delay).\end{tabular}                                     \\ 
%		\vspace*{2mm}
%		$\Theta^h_N$      & \begin{tabular}[c]{@{}l@{}}Number of time slots between the initial\\ collision and the successful transmission of \\ a certain device, provided that it transmitted \\ at the level $h$.\end{tabular}   \\
%		\vspace*{2mm}
%		$\Omega^h_N$      & \begin{tabular}[c]{@{}l@{}}Number of time slots between the first slot \\ transmitted at the level $h$ and the slot of \\ successful transmission of the focused device.\end{tabular}\\
%		\vspace*{2mm}
%		$\mathcal{L}^h_N$ & Number of nodes at the level $h$.                                                                         \\ \bottomrule
%	\end{tabular}
%\end{table}
